Learning to Execute Programs with Instruction Pointer Attention Graph Neural Networks

Graph neural networks (GNNs) have emerged as a powerful tool for learning software engineering tasks including code completion, bug finding, and program repair. They benefit from leveraging program structure like control flow graphs, but they are not well-suited to tasks like program execution that require far more sequential reasoning steps than number of GNN propagation steps. Recurrent neural networks (RNNs), on the other hand, are well-suited to long sequential chains of reasoning, but they do not naturally incorporate program structure and generally perform worse on the above tasks. Our aim is to achieve the best of both worlds, and we do so by introducing a novel GNN architecture, the Instruction Pointer Attention Graph Neural Networks (IPA-GNN), which achieves improved systematic generalization on the task of learning to execute programs using control flow graphs. The model arises by considering RNNs operating on program traces with branch decisions as latent variables. The IPA-GNN can be seen either as a continuous relaxation of the RNN model or as a GNN variant more tailored to execution. To test the models, we propose evaluating systematic generalization on learning to execute using control flow graphs, which tests sequential reasoning and use of program structure. More practically, we evaluate these models on the task of learning to execute partial programs, as might arise if using the model as a heuristic function in program synthesis. Results show that the IPA-GNN outperforms a variety of RNN and GNN baselines on both tasks.

==> scratch.tex <==

IPA-GNN from /cns/oz-d/home/dbieber/learned_interpreters/13660585/5-bs=1,tbs=32,m=1.0,nl=-1,hs=300,acr=T,ad=F,ag=F,iwce=F,n=IPAGNN,ub=T,uce=F,ui=T,up=T,upe=F,n=gnn-relaxed-rnn,ugb=T,lr=0.0003,m=supervised
I0603 13:27:35.945112   87103 length_generalization.py:404] IPA-GNN & 0.43822222222222224
I0603 13:27:36.019846   87103 length_generalization.py:403] NoControl from /cns/oz-d/home/dbieber/learned_interpreters/13660585/10-bs=1,tbs=32,m=1.0,nl=-1,hs=200,acr=T,ad=F,ag=F,iwce=F,n=NoControl,ub=F,uce=T,ui=F,up=F,upe=T,n=gnn-relaxed-rnn,ugb=T,lr=0.0001,m=supervised
I0603 13:27:36.020018   87103 length_generalization.py:404] NoControl & 0.0044444444444444444
I0603 13:27:36.055493   87103 length_generalization.py:403] NoExecute from /cns/oz-d/home/dbieber/learned_interpreters/13660585/21-bs=1,tbs=32,m=1.0,nl=-1,hs=300,acr=F,ad=T,ag=T,iwce=T,n=NoExecute,ub=T,uce=F,ui=T,up=T,upe=F,n=gnn-relaxed-rnn,k=GRU,ugb=T,lr=0.0003,m=supervised
I0603 13:27:36.055677   87103 length_generalization.py:404] NoExecute & 0.15466666666666667
I0603 13:27:36.092026   87103 length_generalization.py:403] GGNN from /cns/oz-d/home/dbieber/learned_interpreters/13660585/26-bs=1,tbs=32,m=1.0,nl=-1,hs=200,acr=F,ad=T,ag=T,iwce=T,n=GGNN,ub=F,uce=T,ui=F,up=F,upe=T,n=gnn-relaxed-rnn,k=GRU,ugb=T,lr=0.0001,m=supervised
I0603 13:27:36.092208   87103 length_generalization.py:404] GGNN & 0.02666666666666667
I0603 13:27:36.129378   87103 length_generalization.py:403] Line-by-Line RNN from /cns/oz-d/home/dbieber/learned_interpreters/13660585/37-bs=128,tbs=32,m=1.0,hs=300,n=rnn,ugb=F,lr=0.0003,m=supervised
I0603 13:27:36.129564   87103 length_generalization.py:404] Line-by-Line RNN & 0.26724910394265233
I0603 13:27:36.167388   87103 length_generalization.py:403] Trace RNN from /cns/oz-d/home/dbieber/learned_interpreters/13686382/2-bs=128,r=trace,tbs=32,m=1.0,hs=200,n=rnn,ugb=F,lr=0.0001,m=supervised
I0603 13:27:36.167560   87103 length_generalization.py:404] Trace RNN & 0.37387992831541217


































































Differentiable relaxation has been used broadly.
Gumbel softmax reparameterization permits differentiating through discrete latent variables \cite{jang2016categorical-reparameterization-with-gumbel-softmax}.

Several works investigate different dimensions of ``learning to execute''.
The task is introduced by \cite{learning-to-execute}.
\cite{nalu} finds a new nonlinearity that generalizes well for addition and multiplication. \cite{neural-code-fusion} uses the task of branch prediction and shows it produces useful program embeddings for a downstream task.





\DANNY{Need a related work section
\begin{itemize}
\item Differentiable relaxation are used broadly:
NTM \cite{neural-turing-machine},
attention \cite{attention-is-all-you-need},
TerpreT \cite{terpret},
neural stack \cite{neural-stack},
differentiable dynamic programming \cite{differentiable-dynamic-programming},
Gumbel softmax \cite{jang2016categorical-reparameterization-with-gumbel-softmax}.
\end{itemize}
}

\todo{Write this section.}
\cite{ggnn}
\cite{neural-program-interpreter}
\cite{neural-turing-machine}
\cite{neural-gpu}
\cite{state-trace-embeddings}
\cite{dypro}
\cite{attention-is-all-you-need}








Graph neural networks have been applied to the study of static analysis
in several recent works
\cite{learning-to-represent-programs-with-graphs,
neural-code-fusion,
great-paper,
lambdanet-type-inference,
deep-learning-type-inference,
javascript-types-gnn}.
\citet{learning-to-represent-programs-with-graphs} uses superimposed control flow and data flow graphs to identify variable misuse and variable misname errors.
\citet{great-paper} constructs a hybrid RNN-GNN model to make further progress on variable misuse by combining sequential processing with program structure analysis.
\citet{lambdanet-type-inference, deep-learning-type-inference, javascript-types-gnn} use graph neural networks
    to perform type inference.
\cite{neural-code-fusion} uses GNNs to perform branch prediction and algorithm classification.

There has been significant interest in program induction with neural networks.
\cite{neural-program-interpreter}
\cite{neural-gpu}
\cite{neural-turing-machine}

Lots of previous work on message passing neural networks:
\cite{quantum-chem-message-passing}
\cite{ggnn}
\cite{semisupervised-gcn}
\cite{graph-attention-networks}









